Unlocking the Capabilities of Thought: A Reasoning Boundary Framework to Quantify and Optimize Chain-of-Thought

Chain-of-Thought (CoT) reasoning has emerged as a promising approach for enhancing the performance of large language models (LLMs) on complex reasoning tasks. Recently, a series of studies attempt to explain the mechanisms underlying CoT, aiming to deepen the understanding of its efficacy. Nevertheless, the existing research faces two major challenges: (1) a lack of quantitative metrics to assess CoT capabilities and (2) a dearth of guidance on optimizing CoT performance. Motivated by this, in this work, we introduce a novel reasoning boundary framework (RBF) to address these challenges. To solve the lack of quantification, we first define a reasoning boundary (RB) to quantify the upper-bound of CoT and establish a combination law for RB, enabling a practical quantitative approach applicable to various real-world CoT tasks. To address the lack of optimization, we propose three categories of RBs. We further optimize these categories with combination laws focused on RB promotion and reasoning path optimization for CoT improvement. Through extensive experiments on 27 models and 5 tasks, the study validates the existence and rationality of the proposed framework. Furthermore, it explains the effectiveness of 10 CoT strategies and guides optimization from two perspectives. We hope this work can provide a comprehensive understanding of the boundaries and optimization strategies for reasoning in LLMs. Our code and data are available at https://github.com/LightChen233/reasoning-boundary.

==> section/mrg.tex <==
\section{Background \& Study Formulation}
Extensive work has shown that when large models handle complex tasks requiring multi-step reasoning, the model's reasoning performance will significantly degrade if the difficulty of a single reasoning step exceeds the model's processing capabilities.

Based on this observation, we believe that for most tasks or models, there is a method that can decompose the reasoning process of complex problems so that the model can effectively handle each reasoning step, thereby achieving its theoretical reasoning capabilities limit.
Based on this idea, we proposed the "feasible reasoning boundary hypothesis".
Specifically, this assumption can be defined as:

\noindent \textbf{Assumption 1:} For a specific task and model, in the thinking chain reasoning process, a single reasoning step has a reasoning limit, that is, the maximum feasible reasoning boundary. reasoning beyond this boundary cannot be performed correctly.
And, If each step of the thinking chain satisfies the maximum feasible reasoning boundary, such a thinking chain can be considered feasible (that is, a feasible thinking chain), otherwise the correct answer cannot be obtained.

Formally, for task $t \in \mathcal{T}$ and model $m \in \mathcal{M}$, when the large model generates a thinking chain of $N$ steps of reasoning $\mathcal{S} = \{\mathcal{S}_i\}^N_{i=1}$, each step $\mathcal{S}_i$ contains an inference conclusion $\mathcal{C}_i \in \mathcal{S}_i$ . For each step of reasoning, there is an ideal correct reasoning conclusion $\hat{\mathcal{C}}_i$. Then the maximum feasible reasoning boundary hypothesis can be formalized as the following conditions:
\begin{equation}
	\label{eq:max_available}
	\forall t \in \mathcal{T}, \forall m \in \mathcal{M}, 
	P(\mathcal{C}_i = \hat{\mathcal{C}}_i |\mathcal{S}_i,t, m) \leq \mathcal{G} (t, m),\  
\end{equation}
where $P(\mathcal{C}_i = \hat{\mathcal{C}}_i |\mathcal{S}_i, t, m)$ represents the given task $t$, model $m$ and current thinking Under the condition of chain step $\mathcal{S}_i$, the model's inference conclusion $\mathcal{C}_i$ is equal to the probability of the correct inference conclusion $\hat{\mathcal{C}}_i$. $\delta(t, m)$ is a threshold related to task $t$ and model $m$, used to determine whether the model's reasoning ability on the task has reached a predetermined upper limit.


\noindent \textbf{Theory 2:} For different abilities, the combined ability satisfies the weighted harmonic average of each basic ability.

\noindent \textit{Proof sketch.} First of all, we define a combined RB $f(x, y)$. When $y\rightarrow +\infty$, it means that the combined RB is not limited by $y$, then the combined reasoning boundary is completely the reasoning boundary of $x$. Similarly, when $x\rightarrow +\infty$, the combined reasoning boundary is completely the reasoning boundary of $y$.

Therefore, we define the combined RB as is the sum of two meta-RB $f(x, +\infty)$ and $f(+\infty, y)$, then we can get condition:
\begin{equation}
	f(x, y) = f(x, +\infty) + f(+\infty, y) \wedge f(+\infty, +\infty) = +\infty
\end{equation}


Since Taylor expansion cannot be performed on infinity and the function needs to converge, we set $x = \frac{1}{t_1}+b_1$ and $y = \frac{1}{t_2}+b_2$ and $\frac{1}{f(x, y)} = g(t_1, t_2)$, then we can get:
\begin{equation}
	g(t_1, t_2) = g(t_1, 0) + g(0, t_2).
\end{equation}

According to Taylor expansion formula, we can get:
\begin{align}
	g(t_1, t_2)&=\lim\limits_{t_2\rightarrow 0} (\sum_{i=0}^{+\infty}N_{1i}t_1^{i}+ \sum_{i=0}^{+\infty}N_{2i}t_2^{i}) + \lim\limits_{t_1\rightarrow 0}(\sum_{i=0}^{+\infty}N_{1i}t_1^{i}+ \sum_{i=0}^{+\infty}N_{2i}t_2^{i})\\
	\sum_{i=0}^{+\infty}N_{1i}t_1^{i}+ \sum_{i=0}^{+\infty}N_{2i}t_2^{i} &= \sum_{i=0}^{+\infty}N_{1i}t_1^{i}+ \sum_{i=0}^{+\infty}N_{2i}t_2^{i} + N_{10} + N_{20}
\end{align}
Therefore $N_{10}+N_{20}=0$. Then, we can further conclude:
\begin{align}
	g(t_1, t_2)& = \sum_{i=0}^{+\infty}N_{1i}t_1^{i}+ \sum_{i=0}^{+\infty}N_{2i}t_2^{i}\\
	&=N_{10} + N_{11} t_1 + \mathcal{O}(t_1)  + N_{20} + N_{21} t_2 +\mathcal{O}(t_2) \\
& \approx N_{11} t_1  + N_{21} t_2
\end{align}
Then the original formula is expressed as:
\begin{equation}
	f(x, y) \approx \frac{1}{\frac{N_{11}}{x-b_1} + \frac{N_{21}}{y-b_2}} \label{eq:combine-proof}
\end{equation}


\noindent \textbf{Theory 2.1:} We believe that the part with an accuracy greater than 0.9 is a fully feasible inference boundary. This part has a high degree of confidence and the model can effectively grasp the performance of this part.

\noindent \textbf{Theory 2.2:} We believe that the part with an accuracy less than 0.1 is a fully feasible inference boundary. This part has a low degree of confidence and the model can never grasp the performance of this part.


\noindent \textbf{Theory 2.3:} We believe that the part with an accuracy greater than 0.1 but less than 0.9 is a partial feasible inference boundary. This part of the model requires repeated thinking or more clear information to solve the problem.
